Salient Information Prompting to Steer Content in Prompt-based Abstractive Summarization

Large language models (LLMs) can generate fluent summaries across domains using prompting techniques, reducing the need to train models for summarization applications. However, crafting effective prompts that guide LLMs to generate summaries with the appropriate level of detail and writing style remains a challenge. In this paper, we explore the use of salient information extracted from the source document to enhance summarization prompts. We show that adding keyphrases in prompts can improve ROUGE F1 and recall, making the generated summaries more similar to the reference and more complete. The number of keyphrases can control the precision-recall trade-off. Furthermore, our analysis reveals that incorporating phrase-level salient information is superior to word- or sentence-level. However, the impact on hallucination is not universally positive across LLMs. To conduct this analysis, we introduce Keyphrase Signal Extractor (SigExt), a lightweight model that can be finetuned to extract salient keyphrases. By using SigExt, we achieve consistent ROUGE improvements across datasets and open-weight and proprietary LLMs without any LLM customization. Our findings provide insights into leveraging salient information in building prompt-based summarization systems. We release our code at \url{https://github.com/amazon-science/SigExt}

==> misc/result-fewshot-1k.tex <==
\begin{table*}[tb]
\centering
\scriptsize
\begin{tabular}{cccccccccc}
\toprule
                &                 & \multicolumn{4}{c}{\textbf{CNN}}                                                & \multicolumn{4}{c}{\textbf{ArXiv}}                                                        \\\cmidrule(lr){3-6}\cmidrule(lr){7-10}
\textbf{Method} & \textbf{\#examples}& \textbf{R-1}         & \textbf{R-2}         & \textbf{R-L}         & \textbf{KW-R}        & \textbf{R-1}         & \textbf{R-2}         & \textbf{R-L}         & \textbf{KW-R}        \\\midrule
Flan-T5-Large         & 1000            & 40.4 (±0.4)          & 17.2 (±0.4)          & 37.5 (±0.4)          & 39.6 (±0.5)          & 41.3 (±0.4)          & \textbf{15.0 (±0.4)} & 37.0 (±0.3)          & 30.8 (±1.2)          \\
+ \ours         & 1000            & \textbf{42.1 (±0.4)} & \textbf{18.4 (±0.5)} & \textbf{39.0 (±0.6)} & \textbf{42.2 (±1.1)} & \textbf{43.3 (±0.7)} & 14.8 (±0.5)          & \textbf{39.0 (±0.7)} & \textbf{34.8 (±0.6)} \\\cmidrule(lr){1-1}
Pegasus-Large         & 1000            & 40.6 (±0.2)          & 17.3 (±0.4)          & 37.5 (±0.3)          & 38.9 (±0.4)          & 40.5 (±0.4)          & 12.8 (±0.5)          & 36.1 (±0.3)          & 28.0 (±0.5)          \\
+ \ours         & 1000            & \textbf{41.8 (±0.7)} & \textbf{17.8 (±1.0)} & \textbf{38.5 (±0.6)} & \textbf{41.0 (±0.4)} & \textbf{40.8 (±0.1)} & \textbf{12.9 (±0.2)} & \textbf{36.5 (±0.2)} & \textbf{32.1 (±1.2)} \\\midrule
Pegasus-Large         & Full            & 44.17                & 21.47                & 41.11                &                      & 44.21                & 16.95                & 38.83                &                      \\
BART-Large            & Full            & 44.16                & 21.28                & 40.90                &                      & 46.54                & 18.82                & 42.00                &                     \\\bottomrule

\end{tabular}
\caption{Effectiveness of \ours using SFT with 1000 samples. We show performance of Pegasus and BART SFT on full dataset as a reference. }
\label{tab:res_flan_1k}
\end{table*}




==> misc/result-fewshot-delta.tex <==
\begin{table}[htb]
\centering\scriptsize
\begin{tabular}{lccccc}
\toprule
\textbf{}       & \textbf{}       & \multicolumn{2}{c}{\textbf{CNN}} & \multicolumn{2}{c}{\textbf{ArXiv}}          \\\cmidrule(lr){3-4}\cmidrule(lr){5-6}
\textbf{Method} & \textbf{\#examples}& \textbf{R-1}        & \textbf{KW-R}        & \textbf{R-1}                & \textbf{KW-R} \\\midrule
Flan &&&&\\
+\gpours  & 32              & +0.7                & +3.1                 & +0.4                        & +1.7          \\
+\gpours  & 128             & +0.6                & +1.6                 & +0.5                        & +3.9          \\
+\ours    & 1000            & +1.7                & +2.6                 & +2.0                        & +4.0          \\\midrule
Pegasus &&&&\\
+\gpours & 32              & +0.8                & +1.2                 & \underline{\color[HTML]{FF0000} -0.3} & +1.2          \\
+\gpours & 128             & +1.1                & +2.6                 & +0.7                        & +1.0          \\
+\ours & 1000            & +1.2                & +2.1                 & +0.3                        & +4.1          \\\bottomrule
\end{tabular}
\caption{The performance gain of \ours in SFT settings with different number of examples.}\label{tab:fewshotdelta}
\end{table}

==> misc/result-prompt-structure.tex <==
\begin{table}[htb]
\scriptsize\centering
\begin{tabular}{cccc}
\toprule
                &                   & \textbf{CNN} & \textbf{ArXiv}       \\
\textbf{Method} & \textbf{Position} & \textbf{KW-R}          & \textbf{KW-R}        \\\midrule
Flan T5 + \ours & End               & \textbf{42.2 (±1.1)}   & \textbf{34.8 (±0.6)} \\
Flan T5 + \ours & Begin             & 41.8 (±0.8)            & 34.1 (±1.3)          \\\midrule
Pegasus + \ours & End               & 41.0 (±0.4)            & 32.1 (±1.2)          \\
Pegasus + \ours & Begin             & \textbf{42.1 (±0.7)}   & \textbf{33.5 (±0.7)} \\\bottomrule
\end{tabular}
\caption{Compare the effect of prompt structure in 1000-shot finetuning settings.}\label{tab:prompt-structure}
\end{table}

==> misc/result-zeroshot.tex <==
\begin{table*}[tb]
\centering\scriptsize
\begin{tabular}{lcccccccc}
\toprule
        & \multicolumn{4}{c}{\textbf{CNN/DailyMail}}  & \multicolumn{4}{c}{\textbf{ArXiv}} \\ 
        \cmidrule(lr){2-5}\cmidrule(lr){6-9}
\textbf{Method}  & \textbf{R-1} & \textbf{R-2} & \textbf{R-L} & \textbf{KW-R} & \textbf{R-1} & \textbf{R-2} & \textbf{R-L} & \textbf{KW-R} \\\midrule
Mixtral-7x8B                  & 38.4 (±0.3)  & 13.5 (±0.1)  & 33.6 (±0.2)  & 40.5 (±0.7)   & 42.3 (±0.4)  & 13.9 (±0.3)  & 37.5 (±0.5)  & 33.7 (±0.3)   \\
+ 2-pass              & 38.0 (±0.3) & 13.4 (±0.1) & 33.0 (±0.1) & 39.9 (±0.6) & 41.9 (±0.2) & 13.5 (±0.1) & 37.1 (±0.2) & 34.2 (±0.4) \\\cmidrule(lr){1-1}
+ \gpours                         & \underline{\color[HTML]{FF0000}38.2 (±0.6)}  & 14.0 (±0.5)  & \underline{\color[HTML]{FF0000}33.4 (±0.6)}  & 42.5 (±0.4)   & 42.8 (±0.6)  & 14.3 (±0.4)  & 38.0 (±0.5)  & 36.3 (±0.6)   \\
+ \ours                     & 39.7 (±0.9)  & 15.4 (±0.5)  & 34.8 (±0.8)  & 43.2 (±0.8)   & 43.5 (±0.7)  & 14.9 (±0.4)  & 38.5 (±0.7)  & 37.2 (±0.7)   \\\midrule
Mistral-7B                   & 38.9 (±0.2)  & 14.5 (±0.5)  & 34.5 (±0.3)  & 37.5 (±0.3)   & 41.8 (±0.4)  & 14.1 (±0.3)  & 37.2 (±0.4)  & 30.8 (±0.5)   \\
+ 2-pass              & 38.7 (±0.4) & 14.5 (±0.2) & 34.2 (±0.5) & 39.7 (±0.9) & 41.8 (±0.5) & 13.7 (±0.2) & 37.2 (±0.4) & 33.4 (±0.4) \\\cmidrule(lr){1-1}
+ \gpours                      & 39.5 (±0.2)  & 15.4 (±0.2)  & 35.2 (±0.1)  & 42.6 (±0.6)   & 42.6 (±0.5)  & 14.4 (±0.3)  & 38.2 (±0.6)  & 35.5 (±0.5)   \\
+ \ours                 & 40.9 (±0.4)  & 16.2 (±0.2)  & 36.3 (±0.2)  & 43.6 (±1.2)   & 43.1 (±0.4)  & 14.8 (±0.2)  & 38.6 (±0.4)  & 36.5 (±0.2)   \\\midrule
Falcon-40B                    & 25.7 (±0.5)  & 9.2 (±0.1)   & 23.1 (±0.4)  & 29.2 (±1.4)   & 39.8 (±0.3)  & 13.7 (±0.3)  & 35.7 (±0.2)  & 31.7 (±0.4)   \\
+ 2-pass              & 33.2 (±1.0) & 12.0 (±0.3) & 29.9 (±0.9) & 38.4 (±1.1) & 39.8 (±0.2) & 13.5 (±0.3) & 35.7 (±0.2) & 33.0 (±0.9) \\\cmidrule(lr){1-1}
+ \gpours                     & 31.9 (±0.4)  & 12.0 (±0.2)  & 28.8 (±0.4)  & 37.8 (±1.2)   & 39.9 (±0.4)  & \underline{\color[HTML]{FF0000} 13.6 (±0.3)}  & 35.8 (±0.4)  & 34.2 (±0.5)   \\
+ \ours                     & 33.5 (±0.5)  & 13.0 (±0.2)  & 30.0 (±0.4)  & 38.9 (±1.1)   & 40.4 (±0.2)  & 14.0 (±0.2)  & 36.3 (±0.2)  & 34.3 (±0.9)   \\\midrule
Flan-T5-XXL                   & 33.8 (±0.2)  & 14.7 (±0.1)  & 30.3 (±0.2)  & 33.3 (±0.4)   & 27.3 (±0.9)  & 10.2 (±0.6)  & 24.3 (±0.8)  & 18.2 (±0.7)   \\
+ 2-pass              & 33.9 (±0.1) & 14.2 (±0.1) & 30.1 (±0.2) & 32.6 (±0.3) & 27.0 (±0.7) & 10.2 (±0.7) & 24.0 (±0.7) & 18.7 (±1.2) \\\cmidrule(lr){1-1}
+ \gpours                         & 35.0 (±0.4)  & 15.2 (±0.2)  & 31.3 (±0.4)  & 36.6 (±0.4)   & 31.7 (±0.5)  & 11.2 (±0.4)  & 28.4 (±0.6)  & 26.9 (±0.6)   \\
+ \ours                      & 35.0 (±0.2)  & 15.2 (±0.1)  & 31.4 (±0.1)  & 37.0 (±0.0)   & 32.5 (±0.2)  & 11.7 (±0.2)  & 29.0 (±0.2)  & 27.3 (±0.8)   \\\midrule
\end{tabular}
\vspace{-1ex}
\caption{Performance of \ours \& \gpours on zero-shot summarization using Mixtral-7x8B-Instruct, Mistral-7B-Instruct, Falcon-40B-Instruct, and Flan-T5-XXL. \ours is trained with 1000 examples, while \gpours is not fine-tuned on the dataset. The LLMs are not fine-tuned. We highlight numbers when 1) \gpours is lower than the vanilla model, or 2) \ours is lower than \gpours.}\label{tab:zeroshot}
\vspace{-1ex}
\end{table*}

